MESA Isochrones and Stellar Tracks (MIST) 0: Methods for the construction of stellar isochrones

I describe a method to transform a set of stellar evolution tracks onto a uniform basis and then interpolate within that basis to construct stellar isochrones. The method accommodates a broad range of stellar types, from substellar objects to high-mass stars, and phases of evolution, from the pre-main sequence to the white dwarf cooling sequence. I discuss situations in which stellar physics leads to departures from the otherwise monotonic relation between initial stellar mass and lifetime and how these may be dealt with in isochrone construction. I close with convergence tests and recommendations for the number of points in the uniform basis and the mass between tracks in the original grid required in order to achieve a certain level of accuracy in the resulting isochrones. The programs that implement these methods are free and open-source; they may be obtained from the project webpage.

==> macros/constants.tex <==
%constants
\newcommand{\kB}{\ensuremath{k_\mathrm{B}}} %Boltzmann's constant
\newcommand{\pF}{\ensuremath{p_\mathrm{F}}} %Fermi momentum
\newcommand{\EF}{\ensuremath{\mathcal{E}_\mathrm{F}}} %Fermi energy
\newcommand{\NA}{\ensuremath{N_\mathrm{\!A}}} %Avogadro number
\newcommand{\mb}{\ensuremath{m_\mathrm{u}}} %mean nucleon mas
\newcommand{\me}{\ensuremath{m_\mathrm{e}}} %electron mass
\newcommand{\mpr}{\ensuremath{m_\mathrm{p}}} %proton mass
\newcommand{\mn}{\ensuremath{m_\mathrm{n}}} %neutron mass
\newcommand{\alphaF}{\ensuremath{\alpha_\mathrm{F}}} %Fine structure


==> macros/refer.tex <==
%=======================================================================
%
% formatting.tex --- Formatting Macros
%
%=======================================================================

%References

\newcommand{\lSect}[1]{{\label{sec:#1}}}
\newcommand{\lFig}[1]{{\label{fig:#1}}}
\newcommand{\lEq}[1]{{\label{eq:#1}}}
\newcommand{\lTab}[1]{{\label{tab:#1}}}
\newcommand{\pFig}[1]{{\placefigure{fig:#1}}}
\newcommand{\pTab}[1]{{\placetable{tab:#1}}}
\newcommand{\Tabff}[1]{{\ref{tab:#1}}}
\newcommand{\Tab}[1]{{Table~\Tabff{#1}}}
\newcommand{\Tabs}[1]{{Tables~\Tabff{#1}}}
\newcommand{\TabRange}[2]{{Tables~\Tabff{#1} - \Tabff{#2}}}
\newcommand{\TabTwo}[2]{{Tables~\Tabff{#1} and \Tabff{#2}}}
\newcommand{\pan}[1]{{\textit{#1}}}
\newcommand{\Pan}[1]{{Panel~\pan{#1}}}
\newcommand{\Pans}[1]{{Panels~\pan{#1}}}
\newcommand{\FIGFF}[2]{{\ref{fig:#2}\pan{#1}}}
\newcommand{\Figff}[1]{{\FIGFF{}{#1}}}
\newcommand{\FIG}[2]{{Fig.~\FIGFF{#1}{#2}}}
\newcommand{\Fig}[1]{{\FIG{}{#1}}}
\newcommand{\FigTwo}[2]{{\FIGS{}{#1} and \FIGFF{}{#2}}}
\newcommand{\FIGS}[2]{{Figs.~\FIGFF{#1}{#2}}}
\newcommand{\Figs}[1]{{\FIGS{}{#1}}}
\newcommand{\Figure}[1]{{Figure~\FIGFF{}{#1}}}
\newcommand{\Figures}[1]{{Figures~\FIGFF{}{#1}}}
\newcommand{\Sectff}[1]{{\ref{sec:#1}}}
\newcommand{\Sect}[1]{{\S\Sectff{#1}}}
\newcommand{\Appendix}[1]{{Appendix~\Sectff{#1}}}
\newcommand{\Appendices}[1]{{Appendices~\Sectff{#1}}}
\newcommand{\Sects}[1]{{\S\S\Sectff{#1}}}
\newcommand{\Eqref}[1]{{\ref{eq:#1}}}
\newcommand{\Eqff}[1]{{(\Eqref{#1})}}
\newcommand{\EQ}[1]{{Equation~\Eqff{#1}}}
\newcommand{\Equation}[1]{{Equation~\Eqff{#1}}}
\newcommand{\Eq}[1]{{Eq.~\Eqff{#1}}}
\newcommand{\Eqs}[1]{{Eqs.~\Eqff{#1}}}
\newcommand{\Leg}[1]{{\textit{#1}}}

% formatting macros

\newcommand{\isofont}[1]{{\mathrm{#1}}}
\newcommand{\isomass}[1]{{\ensuremath{\isofont{^{#1}}}}}
\newcommand{\isocharge}[1]{{\ensuremath{\isofont{_{#1}}}}}
\newcommand{\isotope}[3]{{\ensuremath{\isocharge{#1}\isomass{#2}\isofont{#3}}}}
\newcommand{\Solar}[1]{{\ensuremath{\left[\right.}#1\ensuremath{\right.\left]}}}
\newcommand{\I}[2]{{\isotope{}{#1}{#2}}}
\newcommand{\El}[1]{{\I{}{#1}}}
\newcommand{\Rat}[4]{{\I{#1}{#2}/\I{#3}{#4}}}
\newcommand{\SolRatI}[4]{{\Solar{\Rat{#1}{#2}{#3}{#4}}}}
\newcommand{\SolI}[2]{{\Solar{\I{#1}{#2}}}} \newcommand{\SolEl}[1]{{\Solar{\El{#1}}}} 
\newcommand{\Ep}[1]{{\ensuremath{10^{#1}}}}
\newcommand{\E}[1]{{\ensuremath{\powersep\Ep{#1}}}}
\newcommand{\EE}[2]{{\ensuremath{\powersep\Ep{#1#2}}}}

==> macros/vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
% end vectors.tex

